F$^2$ SLAM: Turning Feed-Forward Geometry into Persistent Factors for SLAM

Feed-forward 3D models provide multi-view geometric predictions, while online simultaneous localization and mapping (SLAM) primarily relies on local measurements. Existing combinations often align or fuse feed-forward predictions after inference, rather than representing them as measurements in the persistent SLAM graph. We present F$^2$ SLAM, which instead converts feed-forward geometry directly into optimization-native target-weight measurements attached to a persistent dense factor graph. A high-frequency stream maintains local tracking constraints and graph connectivity, while a low-frequency stream uses multi-view context to selectively refresh measurements on existing edges after a state-consistency check. Both streams constrain the same poses, inverse depths, and camera intrinsics through a single dense bundle adjustment. Extensive experiments show that F$^2$ SLAM achieves the best average trajectory accuracy on three of the four benchmarks in the uncalibrated setting and competitive trajectory accuracy with known calibration on indoor benchmarks, alongside improved dense reconstruction.

==> sec/3_method_before.tex <==

\section{Feed-forward Factor SLAM}
\label{sec:method}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/pipeline.pdf}
    \caption{
    Overview of \ours{}.
    % The high-frequency stream selects keyframes, maintains active pairs, and frequently updates local target-weight measurements.
    % The low-frequency stream forms scheduled keyframe windows and refreshes selected existing factors using multi-view context.
    % Both streams write measurements into the same persistent factor graph, which is jointly optimized by dense bundle adjustment.
    The high-frequency stream selects keyframes, inserts and maintains active edges, and frequently updates their local target-weight measurements.
    The low-frequency stream forms scheduled keyframe windows and refreshes measurements on selected existing edges using multi-view context, without adding new edges.
    Both streams provide measurements to the same persistent factor graph, whose geometric state is jointly optimized by dense bundle adjustment.
    }
    \label{fig:pipeline}
\end{figure}


\subsection{Persistent Factor-Graph Formulation}
\label{sec:formulation}

Existing feed-forward SLAM systems typically treat feed-forward geometry as an external state that must be aligned or fused with the online estimate.
\ours{} instead brings feed-forward geometry directly into the optimizer as dense measurements.
Both feed-forward and tracking evidence therefore constrain the same persistent geometric state through a single dense BA.

% Given an RGB stream $\{I_t\}_{t=1}^{T}$, the system maintains a sequence of selected keyframes:
% \begin{equation}
%     \mathcal{K}_t
%     =
%     \{k_1,\ldots,k_{N_t}\}.
%     \label{eq:keyframe_set}
% \end{equation}
Given an RGB stream $\{I_t\}_{t=1}^{T}$, the system maintains a set of selected keyframe indices:
\begin{equation}
    \mathcal{K}_t
    =
    \{k_1,\ldots,k_{N_t}\}.
    \label{eq:keyframe_set}
\end{equation}
Here, $N_t=|\mathcal{K}_t|$ is the number of keyframes maintained at time $t$, and $k_n$ denotes the frame index of the $n$-th keyframe in temporal order.
Thus, $k_{N_t}$ identifies the latest keyframe in $\mathcal{K}_t$.

The persistent geometric state is:
% \begin{equation}
%     \mathcal{X}_t
%     =
%     \left\{
%         \mathbf{T}_i,
%         \mathbf{d}_i
%     \right\}_{i\in\mathcal{K}_t},
%     \label{eq:state}
% \end{equation}
% \begin{equation}
% \bar{\mathcal{X}}_t
% =
% \left\{\mathbf{T}_i,\mathbf{d}_i\right\}_{i\in\mathcal{K}_t}
% \cup
% \left\{\boldsymbol{\theta}\right\},
% \end{equation}
\begin{equation}
\mathcal{X}_t
=
\left\{\mathbf{T}_i,\mathbf{d}_i\right\}_{i\in\mathcal{K}_t}
\cup
\left\{\boldsymbol{\theta}\right\},
\label{eq:state}
\end{equation}
%where $\mathbf{T}_i\in SE(3)$ is the pose of keyframe $i$, and $\mathbf{d}_i\in\mathbb{R}_{+}^{h\times w}$ is its dense inverse depth map.
%Camera intrinsics $\boldsymbol{\theta}$ may additionally be optimized when they are unknown.
% where $\mathbf{T}_i\in SE(3)$ denotes the camera-to-world pose of keyframe $i$, $\mathbf{d}_i\in\mathbb{R}_{+}^{h\times w}$ is its dense inverse-depth map, and $\boldsymbol{\theta}$ parameterizes the camera intrinsics.
where $\mathbf{T}_i\in SE(3)$ denotes the world-to-camera transformation of keyframe $i$, $\mathbf{d}_i\in\mathbb{R}_{+}^{h\times w}$ is its dense inverse-depth map, and $\boldsymbol{\theta}$ parameterizes the camera intrinsics.

% When the camera calibration is known, $\boldsymbol{\theta}$ is held fixed and omitted from the optimized variable set.
When the camera calibration is known, $\boldsymbol{\theta}$ is held fixed and omitted from the optimized variable set.
We use $\mathcal{X}_t$ for the geometric variables, $\bar{\mathcal{X}}_t$ for their current estimated values, and $\mathcal{X}_t^{*}$ for the result of a BA solve.

The active portion of the persistent factor graph is:
\begin{equation}
    \mathcal{G}_t
    =
    \left(
        \mathcal{K}_t,
        \mathcal{E}_{\mathrm{act}}^t
    \right),
    \label{eq:factor_graph}
\end{equation}
where $\mathcal{E}_{\mathrm{act}}^t$ is the current set of active directed edges. Each edge $(i,j)$ stores a dense target-weight measurement:
\begin{equation}
    \mathcal{M}_{ij}
    =
    \left(
        \mathbf{p}^{*}_{ij},
        \mathbf{w}_{ij}
    \right).
    \label{eq:measurement}
\end{equation}
%For each pixel $\mathbf{p}\in\Omega_i$, $\mathbf{p}^{*}_{ij}(\mathbf{p})$ denotes its target coordinate in keyframe $j$, while $\mathbf{w}_{ij}(\mathbf{p})$ denotes its precision weight.

% For each pixel, $\mathbf{w}_{ij}(\mathbf{p})\in\mathbb{R}_{+}^{2}$ is a learned confidence weight for the two image-coordinate residual components.
% We define:
% \begin{equation}
%     \mathbf{\Lambda}_{ij}(\mathbf{p})
%     =
%     \operatorname{diag}\!\left(\mathbf{w}_{ij}(\mathbf{p})\right).
% \end{equation}

% The pair $\mathcal{M}_{ij}$ is the measurement stored on edge $(i,j)$, while the corresponding dense factor is the residual cost induced by $\mathcal{M}_{ij}$ and the current geometric state.

For each source pixel $\mathbf{p}\in\Omega_i$, where $\Omega_i$ denotes the source-pixel domain, $\mathbf{p}^{*}_{ij}(\mathbf{p})\in\mathbb{R}^{2}$ is its predicted target coordinate in keyframe $j$.
The vector $\mathbf{w}_{ij}(\mathbf{p})\in\mathbb{R}_{+}^{2}$ contains the learned confidence weights for the horizontal and vertical reprojection-residual components.
We define the corresponding diagonal weight matrix as:
\begin{equation}
    \mathbf{\Lambda}_{ij}(\mathbf{p})
    =
    \operatorname{diag}\!\left(\mathbf{w}_{ij}(\mathbf{p})\right).
    \label{eq:confidence_matrix}
\end{equation}

The dense factor compares the target coordinate projected from the current geometric state with the stored target $\mathbf{p}^{*}_{ij}(\mathbf{p})$.
Their difference is the reprojection residual in Eq.~\eqref{eq:dense_ba_residual}, whose components are weighted by $\mathbf{\Lambda}_{ij}(\mathbf{p})$ in the BA objective in Eq.~\eqref{eq:dense_ba_objective}.

This representation provides a common measurement interface for both streams.
The high-frequency stream frequently updates measurements using local temporal evidence, while the low-frequency stream periodically refreshes selected measurements using a wider multi-view context. Only $\mathcal{X}_t$ is optimized, while all feed-forward outputs are used for initialization, alignment, or factor generation.

\subsection{Dual-stream Pair Construction and Factor Generation}
\label{sec:factor_generation}

Following standard visual SLAM practice, incoming frames are selected as keyframes according to their image-space motion relative to the latest keyframe.
The detailed keyframe insertion and low-frequency scheduling rules are provided in Appendix~\ref{app:motion_keyframe}.

% After a new keyframe $k_{N_t}$ is inserted, the high-frequency stream constructs pairs with temporally nearby and geometrically proximal keyframes.
% Let:
% \begin{equation}
%     \mathcal{N}_{\mathrm{high}}(k_{N_t})
%     =
%     \mathcal{N}_{\mathrm{temp}}(k_{N_t})
%     \cup
%     \mathcal{N}_{\mathrm{prox}}(k_{N_t}),
%     \label{eq:high_neighbors}
% \end{equation}
% denote the selected high-frequency neighbors.
After a new keyframe $k_{N_t}$ is inserted, let $\mathcal{N}_{\mathrm{temp}}(k_{N_t})$ and $\mathcal{N}_{\mathrm{prox}}(k_{N_t})$ denote the sets of temporally nearby and geometrically proximal keyframe indices, respectively.
The high-frequency neighbor set is:
\begin{equation}
    \mathcal{N}_{\mathrm{high}}(k_{N_t})
    =
    \mathcal{N}_{\mathrm{temp}}(k_{N_t})
    \cup
    \mathcal{N}_{\mathrm{prox}}(k_{N_t}).
    \label{eq:high_neighbors}
\end{equation}

The newly generated directed pairs are:
% \begin{equation}
%     \mathcal{P}_{\mathrm{high}}^t
%     =
%     \left\{
%         (k_{N_t},j),
%         (j,k_{N_t})
%         \;\middle|\;
%         j\in
%         \mathcal{N}_{\mathrm{high}}(k_{N_t})
%     \right\}.
%     \label{eq:high_pairs}
% \end{equation}
\begin{equation}
    \mathcal{P}_{\mathrm{high}}^t
    =
    \bigcup_{j\in\mathcal{N}_{\mathrm{high}}(k_{N_t})}
    \left\{(k_{N_t},j),(j,k_{N_t})\right\}.
    \label{eq:high_pairs}
\end{equation}

These pairs are inserted into $\mathcal{E}_{\mathrm{act}}^t$, 
% while edges that leave the active optimization region are removed.
while factors exceeding the update-age or capacity limits are retired as inactive factors with their measurements retained for possible reuse in local BA.
Thus, the high-frequency stream constructs and maintains the persistent graph topology.

% In addition to its target-weight measurement $\mathcal{M}_{ij}$, each active edge stores update
% metadata:
% \begin{equation}
%     \mathcal{F}_{ij}
%     =
%     \left(
%         \mathcal{M}_{ij},
%         \ell_{ij},
%         \gamma_{ij}
%     \right),
%     \label{eq:factor_state}
% \end{equation}
% where source label $\ell_{ij}\in\{\mathrm{high},\mathrm{low}\}$ records the latest measurement source, and $\gamma_{ij}\in\{0,1\}$ is a temporary lock flag.
% The factor-state is mutable edge information and is not part of the optimized geometric state.
Each active edge stores a factor-state containing its target-weight measurement and update metadata:
\begin{equation}
    \mathcal{F}_{ij}
    =
    \left(
        \mathcal{M}_{ij},
        \ell_{ij},
        \gamma_{ij}
    \right),
    \label{eq:factor_state}
\end{equation}
Here, $\mathcal{F}_{ij}$ denotes the stored factor-state of edge $(i,j)$, and $\ell_{ij}\in\{\mathrm{high},\mathrm{low}\}$ identifies the source of its current measurement.
The flag $\gamma_{ij}=0$ allows high-frequency measurement updates, whereas $\gamma_{ij}=1$ prevents the high-frequency stream from overwriting the stored measurement.
The tuple $\mathcal{F}_{ij}$ contains edge data rather than additional geometric variables optimized by BA.

% % For each unlocked edge $(i,j)\in\mathcal{E}_{\mathrm{act}}^t$, the high-frequency predictor estimates a dense displacement offset and precision:
% For each unlocked edge $(i,j)\in\mathcal{E}_{\mathrm{act}}^t$ with $\gamma_{ij}=0$, the high-frequency predictor estimates a dense displacement offset and confidence weights:
% \begin{equation}
%     \left(
%         \Delta\mathbf{p}^{\mathrm{high}}_{ij},
%         \mathbf{w}^{\mathrm{high}}_{ij}
%     \right)
%     =
%     \Psi_{\mathrm{high}}
%     \left(
%         I_i,
%         I_j
%     \right).
%     \label{eq:high_prediction}
% \end{equation}
For each unlocked edge $(i,j)\in\mathcal{E}_{\mathrm{act}}^t$, the high-frequency recurrent update predicts a correction to the current reprojection and its confidence weights:
\begin{equation}
\begin{aligned}
    \big(
        \mathbf{h}_{ij}^{+},
        \Delta\mathbf{p}^{\mathrm{high}}_{ij},
        \mathbf{w}^{\mathrm{high}}_{ij}
    \big)
    =
    \Psi_{\mathrm{high}}
    \big(
        \mathbf{h}_{ij},
        \mathbf{x}_i,
        \mathbf{C}_{ij},
        \mathbf{m}_{ij}
    \big).
\end{aligned}
    \label{eq:high_prediction}
\end{equation}
Here, $\mathbf{h}_{ij}$ and $\mathbf{h}_{ij}^{+}$ are the recurrent hidden states before and after the update, $\mathbf{x}_i$ is the source-frame context feature, and $\mathbf{C}_{ij}$ denotes correlation features sampled at the current reprojection.
The motion feature $\mathbf{m}_{ij}$ encodes the geometry-induced flow and the difference between the stored target and the current reprojection.

Here, $\Psi_{\mathrm{high}}$ denotes the high-frequency measurement predictor.

% The edge factor-state is updated as:
% \begin{equation}
%     \mathcal{F}_{ij}
%     \leftarrow
%     \left(
%         \left(
%             \mathbf{p}
%             +
%             \Delta\mathbf{p}^{\mathrm{high}}_{ij},
%             \mathbf{w}^{\mathrm{high}}_{ij}
%         \right),
%         \mathrm{high},
%         0
%     \right).
%     \label{eq:high_factor_update}
% \end{equation}
The predicted correction is added to the current geometric reprojection to construct the target, after which the edge factor-state is updated:
\begin{equation}
\begin{aligned}
    \mathbf{p}^{*,\mathrm{high}}_{ij}(\mathbf{p})
    &=
    \hat{\mathbf{p}}_{ij}
    \left(\mathbf{p};\bar{\mathcal{X}}_t\right)
    +
    \Delta\mathbf{p}^{\mathrm{high}}_{ij}(\mathbf{p}),\\
    \mathcal{F}_{ij}
    &\leftarrow
    \left(
        \left(
            \mathbf{p}^{*,\mathrm{high}}_{ij},
            \mathbf{w}^{\mathrm{high}}_{ij}
        \right),
        \mathrm{high},
        0
    \right).
\end{aligned}
    \label{eq:high_factor_update}
\end{equation}
The constructed target remains fixed during the ensuing BA solve.

These frequently updated factors provide local constraints for online tracking and bundle adjustment.

% Meanwhile, newly inserted keyframes are accumulated for low-frequency inference. Once the scheduling condition is satisfied, the accumulated keyframes form a window:
% \begin{equation}
%     \mathcal{W}_t
%     =
%     \{k_{a_t},\ldots,k_{b_t}\}.
%     \label{eq:low_window}
% \end{equation}
Meanwhile, newly inserted keyframes are accumulated for low-frequency inference. Once inference is triggered by the scheduling rules in Appendix~\ref{app:motion_keyframe}, the accumulated keyframes form a window:
\begin{equation}
    \mathcal{W}_t
    =
    \{k_{a_t},\ldots,k_{b_t}\}.
    \label{eq:low_window}
\end{equation}
Here, $a_t$ and $b_t$ index the first and last keyframes in the scheduled window.

The window does not define an independent submap or a separate factor graph.
%Instead, it selects existing active pairs whose endpoints both lie inside the window:
Instead, it provides a wider multi-view context for refreshing measurements on selected active edges:
\begin{equation}
    % \mathcal{P}_{\mathrm{low}}^t
    % =
    % \left\{
    %     (i,j)\in\mathcal{E}_{\mathrm{act}}^t
    %     \;\middle|\;
    %     i,j\in\mathcal{W}_t
    % \right\}.
    \mathcal{P}_{\mathrm{low}}^t
    \subseteq
    \left\{
    (i,j)\in\mathcal{E}_{\mathrm{act}}^t
    \;\middle|\;
    i,j\in\mathcal{W}_t,\ i\neq j
    \right\}.
    \label{eq:low_pairs}
\end{equation}
%Therefore, the high-frequency stream constructs the graph topology, whereas the low-frequency window determines which existing factors are eligible for multi-view refresh.

% Thus, the high-frequency stream maintains the graph topology, while the low-frequency stream conditions its measurement predictions on a broader keyframe window. We refer to the resulting measurements as multi-view-context factors.
The low-frequency stream therefore uses the window as multi-view context to refresh measurements on existing edges. We refer to the corresponding dense factors as multi-view-context factors.

Given $\mathcal{W}_t$, the low-frequency stream extracts multi-view features:
\begin{equation}
    \{\mathbf{H}_i\}_{i\in\mathcal{W}_t}
    =
    \mathrm{MVTrans}
    \left(
        \{
            E_{\mathrm{DINO}}(I_i)
        \}_{i\in\mathcal{W}_t}
    \right).
    \label{eq:low_features}
\end{equation}
Here, $E_{\mathrm{DINO}}$ is the DINO image-feature encoder, $\mathrm{MVTrans}$ aggregates its features across the keyframes in $\mathcal{W}_t$, and $\mathbf{H}_i$ is the resulting multi-view feature representation for keyframe $i$.

% Window-level depth and pose predictions derived from these features are used only for initialization and gauge alignment.
When enabled, gauge-aligned poses and depths initialize the shared state before pair selection and validation, but do not directly modify the predicted flow targets.

% For each selected pair $(i,j)\in\mathcal{P}_{\mathrm{low}}^t$, the low-frequency factor head predicts a dense displacement offset and confidence:
% \begin{equation}
%     \left(
%         \Delta\mathbf{p}^{\mathrm{low}}_{ij},
%         \mathbf{c}^{\mathrm{low}}_{ij}
%     \right)
%     =
%     H_{\mathrm{factor}}
%     \left(
%         \mathbf{H}_i,
%         \mathbf{H}_j
%     \right).
%     \label{eq:low_factor_prediction}
% \end{equation}
For each selected pair $(i,j)\in\mathcal{P}_{\mathrm{low}}^t$, the Flow3r-based factor generator constructs a dense flow field and confidence on the BA grid:
\begin{equation}
    \left(
        \mathbf{f}^{\mathrm{low}}_{ij},
        \mathbf{c}^{\mathrm{low}}_{ij}
    \right)
    =
    H_{\mathrm{factor}}
    \left(\mathbf{H}_i,\mathbf{H}_j\right).
    \label{eq:low_factor_prediction}
\end{equation}
Here, $H_{\mathrm{factor}}$ includes prediction decoding and conversion to the common BA grid.
The field $\mathbf{f}^{\mathrm{low}}_{ij}$ denotes the full source-to-target displacement in BA pixel coordinates, rather than a correction to the current geometric reprojection.

% Here, $H_{\mathrm{factor}}$ denotes the low-frequency factor-prediction head, and $\mathbf{c}^{\mathrm{low}}_{ij}$ is its predicted confidence.
The confidence vector $\mathbf{c}^{\mathrm{low}}_{ij}$ has two identical components derived from a scalar confidence gate, yielding equal weights for the horizontal and vertical residuals.

% The predictions are converted into a candidate target-weight measurement:
% \begin{equation}
% \begin{aligned}
%     \mathbf{p}^{*,\mathrm{low}}_{ij}(\mathbf{p})
%     &=
%     \mathbf{p}
%     +
%     \Delta\mathbf{p}^{\mathrm{low}}_{ij}(\mathbf{p}),
%     \qquad
%     \mathbf{w}^{\mathrm{low}}_{ij}
%     &=
%     \eta_{\mathrm{low}}
%     \mathbf{c}^{\mathrm{low}}_{ij},
% \end{aligned}
%     \label{eq:low_target_weight}
% \end{equation}
% % where $\eta_{\mathrm{low}}$ controls the contribution of the low-frequency measurement.
% where $\eta_{\mathrm{low}}$ scales the predicted confidence $\mathbf{c}^{\mathrm{low}}_{ij}$ to obtain the low-frequency measurement weight $\mathbf{w}^{\mathrm{low}}_{ij}$.
The candidate target-weight measurement is constructed as:
\begin{equation}
\begin{aligned}
    \mathbf{p}^{*,\mathrm{low}}_{ij}(\mathbf{p})
    &=
    \mathbf{p}
    +
    \mathbf{f}^{\mathrm{low}}_{ij}(\mathbf{p}),\\
    \mathbf{w}^{\mathrm{low}}_{ij}
    &=
    \eta_{\mathrm{low}}
    \mathbf{c}^{\mathrm{low}}_{ij}.
\end{aligned}
    \label{eq:low_target_weight}
\end{equation}
Here, the source coordinate and flow are expressed on the same BA grid, and $\eta_{\mathrm{low}}$ scales the low-frequency confidence.

We denote the resulting candidate as:
\begin{equation}
    \mathcal{M}^{\mathrm{low}}_{ij}
    =
    \left(
        \mathbf{p}^{*,\mathrm{low}}_{ij},
        \mathbf{w}^{\mathrm{low}}_{ij}
    \right).
    \label{eq:low_candidate_measurement}
\end{equation}

These candidates are not written into the graph immediately.
% Their compatibility with the current SLAM state is first evaluated by the gating procedure described in~\cref{sec:graph_update}.
% Accepted candidates refresh the corresponding factor-states, while rejected candidates leave the existing high-frequency measurements unchanged.

% \subsection{State-Consistent Factor Refresh}
% \label{sec:graph_update}
% Their compatibility with the current SLAM state is first evaluated by the state-consistent validation and refresh procedure described in~\cref{sec:graph_update}.
% Accepted candidates refresh the corresponding factor-states, while rejected candidates leave the existing measurements unchanged.

\subsection{State-Consistent Low-Frequency Factor Refresh}
\label{sec:graph_update}

Accepted candidates refresh the corresponding factor-states, while rejected candidates leave the existing measurements unchanged.
% Low-frequency predictions may be unreliable under occlusion, limited overlap, or imperfect gauge alignment.
% We therefore validate each candidate measurement against the current optimized SLAM state before updating the persistent graph.
Low-frequency predictions may be unreliable under occlusion or limited overlap.
We therefore validate each candidate measurement against the current SLAM state before updating the persistent graph.

For each candidate edge $(i,j)\in\mathcal{P}_{\mathrm{low}}^t$, we compute the reprojection residual:
\begin{equation}
    \mathbf{e}_{ij}^{\mathrm{low}}(\mathbf{p})
    =
    \hat{\mathbf{p}}_{ij}
    \left(
        \mathbf{p};
        \bar{\mathcal{X}}_t
    \right)
    -
    \mathbf{p}_{ij}^{*,\mathrm{low}}(\mathbf{p}),
    \label{eq:low_candidate_residual}
\end{equation}
where $\hat{\mathbf{p}}_{ij}(\mathbf{p};\bar{\mathcal{X}}_t)$ is the target coordinate induced by the current pose and inverse-depth estimates.

% A candidate is accepted when it contains sufficient valid correspondences and its confidence-weighted reprojection error is below a threshold:
% \begin{equation}
%     (i,j)\in\mathcal{S}_{\mathrm{low}}^t
%     \iff
%     r_{\mathrm{sup}}^{ij}
%     \geq
%     \tau_{\mathrm{sup}}
%     \quad\text{and}\quad
%     \bar{e}_{ij}^{\mathrm{low}}
%     \leq
%     \tau_{\mathrm{geo}},
%     \label{eq:accepted_low_edges}
% \end{equation}
% where $r_{\mathrm{sup}}^{ij}$ is the valid-support ratio and $\bar{e}_{ij}^{\mathrm{low}}$ is the confidence-weighted mean residual.
For candidates satisfying $\bar c_{ij}>\tau_{\mathrm{conf}}$,
$r_{\mathrm{in}}^{ij}\geq\tau_{\mathrm{in}}$, and
$N_{\mathrm{in}}^{ij}>0$, the acceptance rule is:
\begin{equation}
    (i,j)\in\mathcal{S}_{\mathrm{low}}^t
    \iff
    r_{\mathrm{sup}}^{ij}\geq\tau_{\mathrm{sup}}
    \quad\text{and}\quad
    s_{ij}\geq\tau_{\mathrm{score}},
    \label{eq:accepted_low_edges}
\end{equation}
where
$s_{ij}=
\bar c_{ij}r_{\mathrm{in}}^{ij}
\sqrt{\max(r_{\mathrm{sup}}^{ij},10^{-6})}
/(1+\bar e_{ij}^{\mathrm{low}})$.
Support consists of geometrically valid pixels with confidence above
$\tau_{\mathrm{conf}}$; inliers additionally satisfy
$\|\mathbf{e}_{ij}^{\mathrm{low}}(\mathbf{p})\|_2<\tau_{\mathrm{geo}}$.
Here, $r_{\mathrm{sup}}^{ij}$ is the support fraction of the full grid,
$r_{\mathrm{in}}^{ij}$ is the inlier fraction of the support,
and $N_{\mathrm{in}}^{ij}$ is the inlier count.
The quantities $\bar c_{ij}$ and $\bar e_{ij}^{\mathrm{low}}$ denote
the mean support confidence and the unweighted mean inlier residual
magnitude, respectively.
All statistics are evaluated on the $1/8$-resolution grid.

For each accepted edge, the low-frequency target-weight measurement refreshes the existing factor-state:
\begin{equation}
    \mathcal{F}_{ij}
    \leftarrow
    \left(
        \mathcal{M}_{ij}^{\mathrm{low}},
        \mathrm{low},
        1
    \right),
    \qquad
    (i,j)\in\mathcal{S}_{\mathrm{low}}^t.
    \label{eq:low_factor_state_update}
\end{equation}

% The temporary lock prevents the accepted measurement from being immediately overwritten by the high-frequency stream.
Once accepted, the low-frequency measurement is protected from high-frequency updates for the remaining lifetime of the factor.
Rejected candidates leave the existing factor-state unchanged.

% This operation only refreshes the measurement of an existing edge.
Accepted candidates refresh the target-weight measurements on existing edges, without changing the graph topology or introducing a separate geometric state.
% It neither changes the graph topology nor directly overwrites poses, inverse depths, or camera intrinsics. All accepted measurements are subsequently optimized in the same persistent dense bundle adjustment.


\subsection{Dense Bundle Adjustment}
\label{sec:dense_ba}

% After factor-state gating, \ours{} jointly refines the persistent geometric state using dense bundle adjustment.
% The backend is agnostic to the source of each measurement.
% For every active edge, it only reads the current target coordinate and precision weight:
\ours{} jointly refines the persistent geometric state using dense bundle adjustment with the measurements selected for the current BA solve.
The backend is agnostic to the source of each measurement.
For every edge in $\mathcal{E}_{\mathrm{BA}}^t$, it only reads the current target coordinate and confidence weights:
\begin{equation}
    \mathcal{M}_{ij}
    =
    \left(
        \mathbf{p}^{*}_{ij},
        \mathbf{w}_{ij}
    \right).
    \label{eq:ba_measurement}
\end{equation}

The source label $\ell_{ij}$ and update lock flag $\gamma_{ij}$ control factor-state updates but do not enter the BA objective.

For a source pixel $\mathbf{p}\in\Omega_i$, the current state predicts its location in keyframe $j$ as:
% \begin{equation}
%     \hat{\mathbf{p}}_{ij}
%     \left(
%         \mathbf{p};
%         \mathcal{X}_t
%     \right)
%     =
%     \pi_{\boldsymbol{\theta}}
%     \left(
%         \mathbf{T}_{j}^{-1}
%         \mathbf{T}_{i}
%         \,
%         \pi_{\boldsymbol{\theta}}^{-1}
%         \left(
%             \mathbf{p},
%             \mathbf{d}_i(\mathbf{p})
%         \right)
%     \right),
%     \label{eq:dense_ba_projection}
% \end{equation}
\begin{equation}
    \hat{\mathbf{p}}_{ij}
    \left(\mathbf{p};\mathcal{X}_t\right)
    =
    \pi_{\boldsymbol{\theta}}
    \left(
        \mathbf{T}_{j}\mathbf{T}_{i}^{-1}
        \,
        \pi_{\boldsymbol{\theta}}^{-1}
        \left(\mathbf{p},\mathbf{d}_i(\mathbf{p})\right)
    \right),
    \label{eq:dense_ba_projection}
\end{equation}

where $\mathbf{T}_i$ and $\mathbf{d}_i$ denote the pose and dense inverse depth of keyframe $i$, respectively.
The camera intrinsics $\boldsymbol{\theta}$ are fixed when the calibration is known and are otherwise optimized jointly with the geometric state.

% The corresponding target-coordinate residual is:
The corresponding reprojection residual is:
\begin{equation}
    \mathbf{r}_{ij}
    \left(
        \mathbf{p};
        \mathcal{X}_t
    \right)
    =
    \hat{\mathbf{p}}_{ij}
    \left(
        \mathbf{p};
        \mathcal{X}_t
    \right)
    -
    \mathbf{p}^{*}_{ij}(\mathbf{p}).
    \label{eq:dense_ba_residual}
\end{equation}
Here, $\mathcal{E}_{\mathrm{BA}}^t$ contains the active factors and
any recent inactive factors selected for the current BA solve.

% Using the precision weight stored on each edge, the persistent state is optimized:
Using the confidence-weight matrix $\mathbf{\Lambda}_{ij}$ defined in Eq.~\eqref{eq:confidence_matrix}, the persistent state is optimized:
\begin{equation}
\begin{aligned}
\mathcal{X}_t^{*}
=
\arg\min_{\mathcal{X}_t} \,
% & \sum_{(i,j)\in\mathcal{E}_{\mathrm{act}}^t}
&\sum_{(i,j)\in\mathcal{E}_{\mathrm{BA}}^t}
\sum_{\mathbf{p}\in\Omega_i}
v_{ij}(\mathbf{p}) \,
\rho \left(
\mathbf{r}_{ij}(\mathbf{p}; \mathcal{X}_t)^{\top}
\mathbf{\Lambda}_{ij}(\mathbf{p})
\mathbf{r}_{ij}(\mathbf{p}; \mathcal{X}_t)
\right) \\
& + \frac{\lambda_d}{2}
\sum_{i\in\mathcal{K}_t}
\| \nabla\mathbf{d}_i \|_2^2
+ \frac{\lambda_{\theta}}{2}
\| \boldsymbol{\theta} - \boldsymbol{\theta}_0 \|_{\mathbf{\Sigma}_{\theta}^{-1}}^2 ,
\end{aligned}
\label{eq:dense_ba_objective}
\end{equation}
where $v_{ij}$ masks invalid correspondences, $\rho$ is a robust penalty, the second term regularizes the dense inverse-depth maps, and the third term constrains the camera intrinsics around the calibration prior $\boldsymbol{\theta}_0$.
The intrinsic term is omitted when calibration is fixed.

% The objective contains one residual for each active edge, regardless of whether its current measurement is generated by the high-frequency stream or accepted from the low-frequency stream.
% An accepted low-frequency prediction only replaces $\mathcal{M}_{ij}$ on the corresponding edge. It does not add another residual or introduce an additional pose, depth, or submap variable.
% Unrefreshed edges retain their current high-frequency measurements.
The objective contains one dense residual term for each edge in $\mathcal{E}_{\mathrm{BA}}^t$.
An accepted low-frequency measurement only replaces the stored measurement on an existing edge, without adding another residual term or introducing a separate geometric state.
Unrefreshed edges retain their current measurements.

Consequently, both streams constrain the same poses, inverse depths, and optional intrinsics through a single BA in the persistent online gauge.
The detailed residual linearization, Gauss--Newton system, and state update rules are provided in Appendix~\ref{app:state_optimization}.


==> sec/4_exper_before.tex <==
\section{Experiments}
\subsection{Experimental Setup}

\input{tabs/tab_tum_traj}
\input{tabs/tab_7scenes_traj}

We evaluate \ours{} on four standard SLAM datasets: TUM RGB-D~\citep{tum}, 7-Scenes~\citep{shotton2013scene}, Replica~\citep{replica}, and KITTI Odometry~\citep{kitti}, covering indoor, outdoor, synthetic, and real-world settings.
Following~\citep{vggtslam}, we use the \texttt{evo} toolkit to Sim(3)-align estimated trajectories and report the root mean square error of absolute trajectory error (ATE RMSE).
Following~\citep{SLAM-Former}, we evaluate dense reconstruction on Replica and 7-Scenes datasets using accuracy (Acc.), completion (Comp.), and Chamfer distance.

We compare against representative classical, learning-based, and feed-forward SLAM methods, including ORB-SLAM2/3~\citep{orbslam2,orbslam3}, LDSO~\citep{ldso}, DROID-SLAM~\citep{droidslam}, DPV-SLAM~\citep{dpvslam}, DPV-SLAM++~\citep{dpvslam}, GO-SLAM~\citep{goslam}, NICER-SLAM~\citep{nicerslam}, MASt3R-SLAM~\citep{mast3rslam}, VGGT-SLAM variants~\citep{vggtslam,vggtslam2,vggtslam++}, and SLAM-Former~\citep{SLAM-Former}, Lingbot-Map~\citep{lingbotmap}, MASt3R~\citep{mast3r}, CUT3R~\cite{cut3r}, Spann3R~\citep{spann3r}, SLAM3R~\citep{slam3r}, and StreamVGGT~\citep{zhuo2025streaming}.
We use the results reported by SLAM-Former as part of the baseline comparison.
All our experiments are performed on a single NVIDIA A100 GPU (40GB VRAM) paired with an AMD EPYC 7542 CPU.
All evaluations use a deterministic inference pipeline without random sampling or seed-dependent operations. Uncalibrated methods do not use ground-truth camera intrinsics.

Unless stated otherwise, \ours{} uses fixed pretrained DROID-Net~\citep{droidslam} and Flow3r~\citep{flow3r} weights on all datasets. 
The low-frequency feed-forward measurements are incorporated into the dense BA backend described in~\cref{sec:method}. 
We use Flow3r poses and depths to initialize the optimization.
Within each calibration setting, the \sotabox{best} and \secondbox{second-best} results are highlighted in green (bold) and orange (underlined), respectively.


\input{tabs/tab_replica_traj}
\input{tabs/tab_kitti_traj}
\input{tabs/tab_replica_recon}
\input{tabs/tab_7scenes_recon}

\subsection{Trajectory Evaluation}

We evaluate trajectory estimation on TUM RGB-D, 7-Scenes, Replica, and KITTI Odometry datasets.
\cref{tab:tum_traj,tab:7scenes_traj,tab:replica_traj,tab:kitti_traj} report the ATE RMSE under the standard evaluation protocol of each benchmark~\citep{vggtslam}. 
Our method achieves three optimal values and one suboptimal value on four datasets in the uncalibrated setting and also achieves competitive results in the calibrated setting.

%In the uncalibrated setting, \ours{} achieves the strongest or competitive average trajectory accuracy across the evaluated benchmarks. Compared with the corresponding VGGT-SLAM variants, it reduces the average ATE by approximately 24--90\% on the indoor datasets and by 54\% on KITTI. The largest margin is observed on Replica, while KITTI provides a complementary long-horizon outdoor setting.

The particularly strong Replica result is related to the high-frequency DROID-Net tracking stream. 
Replica consists of synthetic indoor sequences with stable illumination, limited motion blur, and relatively small inter-frame motion. 
These conditions provide reliable adjacent-frame correspondences, allowing recurrent tracking factors to maintain a strong local geometric estimate. The feed-forward stream then serves as a complementary multi-view correction.
The Replica ablation experiments in \cref{tab:ablation} is consistent with this interpretation.

On TUM RGB-D, \ours{} achieves the best average result among the evaluated uncalibrated methods, and it remains competitive on 7-Scenes while obtaining the best result on several sequences. 
On KITTI, \ours{} substantially improves over uncalibrated foundation-model baselines, although calibrated systems with dedicated loop closure or specialized global optimization remain stronger on some sequences.

The paired \ours{} rows with and without ground-truth intrinsics provide a direct comparison of intrinsic refinement. 
The uncalibrated configuration matches or improves upon the ground-truth-intrinsics configuration across all benchmark averages, with the largest gain on KITTI. 
This observation does not imply that the dataset calibration is incorrect.
Instead, it may reflect a mismatch between nominal intrinsics and the effective image formation model after resizing, cropping, rectification, or different camera-model conventions. 
Joint intrinsic refinement may help absorb such systematic reprojection bias, which is consistent with the improved uncalibrated results.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/recon.pdf}
    \caption{
    Qualitative reconstruction comparison on representative sequences.
    Compared with existing methods, \ours{} recovers more complete scene geometry with fewer artifacts and better preserves fine structures and surface consistency.
    }
    \label{fig:recon}
\end{figure}


\subsection{Reconstruction Evaluation}

We evaluate dense reconstruction on Replica and 7-Scenes datasets. \cref{tab:7scenes_recon,tab:replica_recon} summarize the quantitative results, and \cref{fig:recon} provides qualitative comparisons. 
To ensure fairness, we do not employ any method-specific post-processing techniques, such as confidence-based point filtering~\citep{SLAM-Former}.

% Across the reported reconstruction metrics, \ours{} achieves strong performance on both benchmarks.
%Under comparable final point-cloud budgets, \ours{} achieves the strongest overall reconstruction quality on both benchmarks. 
On Replica, \ours{} obtains the best average accuracy and completion, with a particularly consistent improvement in surface coverage across the evaluated scenes.
On 7-Scenes, it matches the best accuracy while reducing completion and chamfer distance by approximately 50\% and 30\%, respectively, relative to the strongest feed-forward baseline. 

The qualitative results support these quantitative findings. \ours{} recovers more continuous surfaces and fewer missing regions than the compared methods as shown in \cref{fig:recon}. 
Together with the trajectory results, these findings suggest that jointly optimizing local tracking measurements and feed-forward geometric evidence improves both camera consistency and multi-view surface alignment.

\subsection{Ablation}

\subsubsection{Intrinsic Refinement in the Uncalibrated Setting}

In the uncalibrated setting, \ours{} jointly optimizes intrinsics, poses, and inverse depths using both
high-frequency tracking factors and low-frequency feed-forward factors.
This is important because intrinsic errors introduce systematic reprojection biases that cannot be fully absorbed by pose or depth updates alone.
The paired \ours{} rows in \cref{tab:tum_traj,tab:7scenes_traj,tab:replica_traj,tab:kitti_traj} directly compare optimization with and without ground-truth intrinsics.
The self-calibrated configuration matches or improves the ground-truth-intrinsics configuration across all benchmark averages, demonstrating that the unified optimization remains effective without ground-truth camera intrinsics.


% \subsubsection{Ablation on Initialization and Factors}

% \cref{tab:ablation_factor} isolates the effects of feed-forward initialization and persistent factor integration on Replica. 
% Each component individually improves the tracking-only baseline, but their combination yields the best performance across all metrics. 
% Compared with basic tracking, the complete system reduces trajectory error by about 13\% and improves the two reconstruction metrics by 7--12\%.

% Initialization provides a state that is more compatible with the feed-forward geometry, whereas factor integration preserves this information during subsequent optimization. Their combination therefore gives a stronger and more consistent improvement than either component alone, supporting the complementary roles of state initialization and persistent measurement constraints.

\subsubsection{Ablation on Initialization, Factors, Gauge Alignment, and Gating}

\cref{tab:ablation} disentangles the contributions of feed-forward initialization, measurement-level integration, and state-consistent gating on Replica. 
Initialization and factor integration each improve tracking and reconstruction performance, while their combination achieves the best trajectory and reconstruction performance. Compared with basic tracking, the full configuration reduces trajectory error by about 15\% and improves the reconstruction metrics by 7--12\%.

%Removing the gate consistently degrades performance compared with the gated variant, demonstrating the importance of state-consistent admission for reliable feed-forward measurement integration.
Removing gauge alignment mainly degrades reconstruction while leaving trajectory accuracy comparable, indicating that expressing the predicted pose and depth in the current SLAM gauge is important for state-consistent initialization. 
Removing state-consistent gating causes catastrophic degradation under the same configuration, showing that feed-forward predictions cannot be unconditionally written into the persistent graph. 
Together, these results support our design: feed-forward geometry provides complementary initialization and optimization-native measurements, while gauge alignment and state-consistent admission ensure consistent and reliable updates to dense BA.

%These results support the key design of \ours{}: feed-forward geometry serves both as a geometry-aware initialization and as an optimization-native measurement source, while state-consistent admission ensures that only reliable measurements refresh the persistent dense BA.




==> tabs/copy.tex <==
\begin{table}[htbp]
\centering
\caption{Reconstruction accuracy and completion on Replica. Lower is better. Best results are shown in bold.  $+$ denotes the results reported in NICER-SLAM.  $++$ shows the results from SLAM3R. $*$ represented the results from our run.}
\label{tab:results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccc}
\toprule
 & \multicolumn{2}{c}{Room0} & \multicolumn{2}{c}{Room1} & \multicolumn{2}{c}{Room2} & \multicolumn{2}{c}{Office0} & \multicolumn{2}{c}{Office1} & \multicolumn{2}{c}{Office2} & \multicolumn{2}{c}{Office3} & \multicolumn{2}{c}{Office4} & \multicolumn{2}{c}{Avg} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17} \cmidrule(lr){18-19}
Method & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. \\
\midrule
DUSt3R$^{++}$ & 3.47 & 2.50 & 2.53 & 1.86 & 2.95 & 1.76 & 4.92 & 3.51 & 3.09 & 2.21 & 4.01 & 3.10 & 3.27 & 2.25 & 3.66 & 2.61 & 3.49 & 2.48 \\
MASt3R$^{++}$ & 4.01 & 4.10 & 3.61 & 3.25 & 3.13 & 2.15 & 2.57 & 1.63 & 12.85 & 8.13 & 3.13 & 1.99 & 4.67 & 3.15 & 3.69 & 2.47 & 4.71 & 3.36 \\
\midrule
NICER-SLAM$^{+}$ & 2.53 & 3.04 & 3.93 & 4.10 & 3.40 & 3.42 & 5.49 & 6.09 & 3.45 & 4.42 & 4.02 & 4.29 & 3.34 & 4.03 & 3.03 & 3.87 & 3.65 & 4.16 \\
DROID-SLAM$^{+}$ & 12.18 & 8.96 & 8.35 & 6.07 & 3.26 & 16.01 & 3.01 & 16.19 & 2.39 & 16.20 & 5.66 & 15.56 & 4.49 & 9.73 & 4.65 & 9.63 & 5.50 & 12.29 \\
DIM-SLAM$^{+}$ & 14.19 & 6.24 & 9.56 & 6.45 & 8.41 & 12.17 & 10.16 & 5.95 & 7.86 & 8.33 & 16.50 & 8.28 & 13.01 & 6.77 & 13.08 & 8.62 & 11.60 & 7.85 \\
Spann3R$^{++}$ & 9.75 & 12.94 & 15.51 & 12.94 & 7.28 & 8.50 & 5.46 & 18.75 & 5.24 & 16.64 & 9.33 & 11.80 & 16.00 & 9.03 & 13.97 & 16.02 & 10.32 & 13.33 \\
GO-SLAM$^{++}$ & / & / & / & / & / & / & / & / & / & / & / & / & / & / & / & / & 3.81 & 4.79 \\
\midrule
SLAM3R$^{++}$ & 3.19 & 2.40 & 3.12 & 2.34 & 2.72 & 2.00 & 4.28 & 2.60 & 3.17 & 2.34 & 3.84 & 2.78 & 3.90 & 3.16 & 4.32 & 3.36 & 3.57 & 2.62 \\
SLAM3R* & 3.59 & 2.59 & 2.82 & 1.95 & 3.22 & 2.29 & 5.07 & 2.85 & 3.45 & 2.41 & 3.64 & 2.50 & 3.66 & 2.58 & 3.29 & 2.40 & 3.59 & 2.45 \\
%CUT3R & 6.09 & 3.09 & 9.89 & 4.55 & 5.77 & 2.66 & 5.23 & 2.46 & 11.60 & 6.94 & 8.00 & 3.16 & 6.12 & 3.09 & 7.46 & 3.05 & 7.52 & 3.62 \\
%StreamVGGT & 9.01 & 4.37 & 12.22 & 4.66 & 5.61 & 2.61 & 6.64 & 3.45 & 5.14 & 2.55 & 12.84 & 7.23 & 12.09 & 6.59 & 15.48 & 6.35 & 9.88 & 4.73 \\
MSt3R-SLAM* & 24.68 & 26.75 & 3.93 & 2.66 & 2.58 & 1.87 & 3.36 & 2.11 & 3.59 & 3.03 & 6.09 & 4.84 & 8.81 & 8.24 & 7.42 & 5.77 & 7.56 & 6.91 \\
VGGT-SLAM & 3.23 & 2.33 & 18.92 & 15.41 & 15.93 & 12.37 & 4.01 & 2.49 & 3.01 & 2.32 & 6.93 & 5.31 & 2.97 & 2.53 & 5.19 & 3.53 & 7.52 & 5.86 \\
%SLAM-Former & 2.40 & 1.86 & 1.79 & 1.35 & 1.83 & 1.39 & 1.84 & 1.37 & 1.70 & 1.28 & 2.44 & 1.67 & 2.36 & 1.89 & 2.38 & 1.70 & 2.09 & 1.56 \\
SLAM-Former* & 3.39 & 2.47 & 2.48 & 1.71 & 2.44 & 1.66 & 2.08 & 1.53 & 1.78 & 1.38 & 3.45 & 2.22 & 2.96 & 2.13 & 3.05 & 2.08 & 2.70 & 1.87 \\
%EC3R-SLAM & 2.07 & 1.63 & 2.90 & 2.03 & 1.93 & 1.57 & 4.06 & 2.48 & 2.17 & 1.69 & 3.41 & 2.43 & 2.51 & 2.08 & 3.52 & 2.66 & 2.82 & 2.07 \\
Ours & 3.13 & 2.26 & 2.59 & 1.66 & 2.46 & 1.67 & 2.30 & 1.48 & 1.79 & 1.31 & 2.58 & 1.69 & 3.27 & 2.13 & 3.21 & 2.10 & 2.67 & 1.74 \\
\bottomrule
\end{tabular}%
}
\end{table}



\begin{table}[t]
\centering
% \small
\caption{Root mean square error (RMSE) of absolute trajectory error (ATE (cm)) on Replica~\citep{straub2019replica}. Lower is better. Best results are shown in bold.}
\label{tab:replica_traj}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccccccc}
\toprule
Method & Uncalib. & R0 & R1 & R2 & O0 & O1 & O2 & O3 & O4 & Avg. \\
\midrule
% \multicolumn{11}{l}{\textit{Calibrated / RGB-D SLAM}} \\
NICER-SLAM~\citep{zhu2024nicer} 
& \xmark  & 1.300 & 1.600 & 1.100 & 2.100 & 3.200 & 2.100 & 1.400 & 2.000 & 1.850 \\
DROID-SLAM~\citep{teed2021droid} 
& \xmark  & 0.300 & 0.100 & 0.300 & 0.300 & 0.400 & 0.300 & 0.500 & 0.400 & 0.325 \\
\textbf{\ours{} (ours)}
& \xmark  & 0.261 & 0.214 & 0.300 & \textbf{0.216} & \textbf{0.311} & \textbf{0.279} & \textbf{0.336} & \textbf{0.363} & \textbf{0.285} \\
\midrule
% \multicolumn{11}{l}{\textit{Uncalibrated / Feed-forward SLAM}} \\
SLAM3R~\citep{liu2025slam3r} 
&\cmark& 4.600 & 5.900 & 5.700 & 11.200 & 6.300 & 6.200 & 5.000 & 8.100 & 6.625 \\
CUT3R~\citep{wang2025continuous} 
&\cmark& 14.500 & 24.300 & 12.700 & 15.900 & 23.000 & 16.200 & 8.800 & 20.400 & 16.975 \\
StreamVGGT~\citep{zhuo2025streaming} 
&\cmark& 11.300 & 16.300 & 7.700 & 7.600 & 7.000 & 18.000 & 15.300 & 16.800 & 12.500 \\
VGGT-SLAM~\citep{maggio2026vggt} 
&\cmark& 3.000 & 16.700 & 8.600 & 4.200 & 6.400 & 9.500 & 3.900 & 4.300 & 7.075 \\
% SLAM-Former~\citep{yuan2025slam} 
% &\cmark& 3.000 & 2.600 & 2.700 & 2.800 & 2.900 & 3.800 & 2.800 & 3.100 & 2.963 \\
\textbf{\ours{} (ours)} 
&\cmark& \textbf{0.222} & \textbf{0.192} & \textbf{0.211} & \textbf{0.196} & \textbf{0.218} & \textbf{0.234} & \textbf{0.216} & \textbf{0.235} & \textbf{0.215} \\
\bottomrule
\end{tabular}
}
\end{table}
